Efficient Timestamping for Sampling-based Race Detection

Dynamic race detection based on the happens before (HB) partial order has now become the de facto approach to quickly identify data races in multi-threaded software. Most practical implementations for detecting these races use timestamps to infer causality between events and detect races based on these timestamps. Such an algorithm updates timestamps (stored in vector clocks) at every event in the execution, and is known to induce excessive overhead. Random sampling has emerged as a promising algorithmic paradigm to offset this overhead. It offers the promise of making sound race detection scalable. In this work we consider the task of designing an efficient sampling based race detector with low overhead for timestamping when the number of sampled events is much smaller than the total events in an execution. To solve this problem, we propose (1) a new notion of freshness timestamp, (2) a new data structure to store timestamps, and (3) an algorithm that uses a combination of them to reduce the cost of timestamping in sampling based race detection. Further, we prove that our algorithm is close to optimal -- the number of vector clock traversals is bounded by the number of sampled events and number of threads, and further, on any given dynamic execution, the cost of timestamping due to our algorithm is close to the amount of work any timestamping-based algorithm must perform on that execution, that is it is instance optimal. Our evaluation on real world benchmarks demonstrates the effectiveness of our proposed algorithm over prior timestamping algorithms that are agnostic to sampling.

==> eval-tsan-old.tex <==
%!TEX root=./main.tex

\subsection{Evaluation on \tsan}


\subsubsection{Evaluation Setup} 
We first describe our experimental and benchmark setup.
% and explain the effects of our vector clock optimizations in the benchmarks under test.


\myparagraph{Benchmarks}{
Since \tsan is known to be a well-engineered tool, 
developed and supported for more than $15$ years primarily by software developers at Google,
we expect that a simple algorithmic improvement like ours, 
without aggressive tuning to cater for crucial low-level performance
details such as cache misses, is likely to be naive and may in fact
hurt performance.
Therefore, for a thorough evaluation of our algorithms,
we resorted to an intensive real-world application
with a diverse workload, instead of running \tsan on small unit tests in public open-source repositories.
Our primary evaluation subject is the MySQL Server 8.0.37, thanks to
its elaborate use of multi-threading and concurrency primitives.
Our suite contains $11$ benchmarks  from 
the BenchBase framework~\cite{DifallahPCC13} that are our compatible with our setup.
Each benchmark comprises of a schema and workload (sequence of queries),
and together the suite provides a good diversity in the execution characteristics,
including runtime characteristics such as expected lock contention.
}

\myparagraph{Build configurations}{
Our primary evaluation goal for this setup is to gauge
the impact of the new timestamping algorithms we introduce here.
Towards this, we compile MySQL in different configurations:
\begin{enumerate*}
    \item \underline{No-TSan (\confNT)}, i.e., compiled without any instrumentation.
    \item \underline{TSan (\confT)}, i.e., compiled with (original) TSan v3.
    \item \underline{Sampling-TSan (\confST)}, i.e., compiled with TSan v3, but only 3\% access events are sampled.
    \item \underline{Sampling-UClock (\confSU)} - compiled with TSan v3 with modified timestamping as in \algoref{smp-upd} and samples 3\% access events.
    \item \underline{Sampling-OrderedList (\confSO)} - compiled with TSan v3 with modified timestamping as in \algoref{algo4} and samples 3\% accesses.
\end{enumerate*}
The configurations \confNT, \confT and \confST serve as baselines for our algorithms (\confSU and \confSO).
% We assess the effectiveness of our proposed algorithms by comparing the benchmark results for \textsf{sampling-tsan} (baseline), \textsf{sampling-u}, and \textsf{sampling-o}.
% We also ran the benchmarks on no-tsan and tsan to measure the performance cost incurred by TSan with and without sampling. 
}

\myparagraph{Implementation and Setup}{
We directly modify the callback functions of TSan (in LLVM's \texttt{compiler-rt})
and modify those for acquire, release, load, store, fork and join events.
We also adapted our algorithms for other synchronization primitives such 
as read locks or atomic store operations with release memory order, as these are used in MySQL.
We also disabled SSE and preemption of slots in TSan v3.
% We remark that on top of normal lock releases and acquires, TSan also needs to provide handlers for various other synchronization primitives such as read locks or atomic store operations with release memory order. We adapted our algorithms to follow the semantics of these primitives in their corresponding handlers. We also disabled SSE and preemption of slots in TSan.
We configured the BenchBase suite to run for 1 hour, using the 
\texttt{SERIALIZABLE} isolation level, with $60$ client threads, 
a rate limit of $10$ million requests, and a 
fixed \texttt{randomSeed} to ensure that all runs, irrespective of their configurations,
processed the same requests. 
The seed for sampling (i.e., those responsible for choosing which events to sample)
are of course not fixed and randomly determined instead.
% For configurations that perform sampling, 
% we use a different seed for the sampler in every run, but use the same set of seeds for all benchmark-build pairs. 
We ran each pair of configuration and benchmark
for $25$ times on AMD EPYC Milan 7713 cluster machines with $128$ CPUs and $64$GB memory.
We turned off race reporting by TSan to avoid the resulting I/O overhead.
% The I/O overhead of bug reporting, we turned it off by adding \texttt{report\_bugs=0} to \texttt{TSAN\_OPTIONS} as suggested in the TSan documentation.
We gathered two statistics from each trial that are representative
of the performance of MySQL in each configuration ---
\begin{enumerate*}[label=(\alph*)]
    \item the \emph{latency} of, i.e., time taken to complete, each query, and,
    \item the overall \emph{throughput} of MySQL during the entire run.
\end{enumerate*}
We report different percentiles of the latency distribution (aggregated over different runs),
since even a single workload comprises of a wide variety of requests, and a fine grained
information about the distribution lends insights into the performance characteristics.
% Throughout each run, we collected the latency (time taken) of every request and the overall throughput (number of requests completed per second) in this period. 
% At the end of each run, we take the various percentiles of the latency distribution, and report the average of these values over all runs for the same benchmark-build pair.
% We consider the various percentiles because each benchmark runs a workload that is composed of a variety of requests which may be completed in a different amount of time.
}

% This figure is not so useful according to reviewer feedback. It is also good to leave more room for the formal statements in earlier statements.
\begin{figure}[t]
\includegraphics[width=1\textwidth]{figures/mysql-latencies.pdf}
\vspace{-0.1 in}
\caption{Percentage of \confSU and \confSO latencies relative to \confST}
\figlabel{mysql-latencies}
\end{figure}

\input{tables/tsan-throughputs}

\subsubsection{Results}
In \figref{mysql-latencies}, we show the latency distribution of queries across all 
configurations that sample events and monitor them using vector clocks, and in
\tabref{tsan-throughputs}, we present the throughput values across all configurations.
A few straightforward observations are in order:
\begin{enumerate}
\item (\underline{\it Benchmark diversity}). We observe that the latencies vary widely across 
the queries of a given workload; see for example the latencies in
\textsf{auctionmark}  ($1.9$k $\mu$s to $1.6$M $\mu$s) in \figref{mysql-latencies}.
Further, the distributions across workloads is also diverse;
compare for example, the 50\%-ile of \textsf{tatp} v/s \textsf{tpcc} on \figref{mysql-latencies};
also compare throughput values in the \confNT baseline (\tabref{tsan-throughputs}) 
for \textsf{tpcc} v/s \textsf{ycsb}.

\item (\underline{\it Overhead due to \tsan}). 
Columns 1 and 2 in \tabref{tsan-throughputs} indicate
that for our subject, MySQL Server, \tsan does add a significant slowdown
as compared to the uninstrumented version. See for example
the benchmark \textsf{twitter}
where the throughput in \confT is $40\times$ lower than the
uninstrumented baseline \confNT.

\item (\underline{\it Effect of sampling}). 
Further, sampling in general does indeed
reduce the overhead induced by the full-fledged 
\tsan in practice (compare Column 3 with Column 4 in \tabref{tsan-throughputs}).
Next, in many cases, our algorithms further 
improve the naive timestamping algorithm in the case of sampling 
(compare Columns 5 and 6 with Column 4).
\end{enumerate}

Let us now dive deeper into individual benchmarks.
% Let us now focus on \figref{mysql-latencies} and evaluate how the
% timestamping algorithms (\confSU) and data structure (\confSO) we propose impact
% the performance of sampling based race detection in the context of different workloads.
In order to determine which benchmarks led to a statistically 
significant change (in terms of latency distribution) over the sampling baseline \confST,
we employed a two-sample t-test with a 5\% significance level, with
results as follows:
\begin{enumerate}
    \item \underline{\textsf{sibench} and \textsf{ycsb}}. For these benchmarks, 
    both \confSU and \confSO
    were determined to perform better than the baseline \confST ---
    \textsf{sibench} shows upto $1.97\times$ improvement in latency
    and $1.32\times$ improvement in aggregated throughput,
    while \textsf{ycsb} shows a consistent  improvement  (close to $2\times$) in latency 
    and throughput.
    The workloads of these benchmarks often involve
    multiple threads accessing the same table record at a high rate, 
    causing high contention on locks that protect these records. 
    In these cases, the overhead of vector clock computations is naturally
    compounded since timestamping further delays the release of locks in the underlying operations.
    As a result, the speedup from our vector clock optimizations is also compounded
    (also compare Columns 5 and 6 with Column 4 in \tabref{tsan-throughputs}).

    \item \underline{\textsf{tatp} and \textsf{twitter}}. For these benchmarks,
    the performance of the configuration \confSU was determined
    to be poorer than \confST or \confSO.
    Upon further profiling, we found that these benchmarks were primarily sparse, but I/O heavy
    with low lock contention.
    Further, these benchmarks often trigger frequent non-mutex synchronizations in MySQL,
    such as the use of atomic stores with release memory order, optimizing
    timestamping for which is beyond the scope of
    our current work. As a consequence, the slowdown incurred due to extra metadata checks and updates 
    instead lead to a marginal slowdown. Such a slowdown is more overwhelming for \confSU as it computes the complete freshness timestamp while \confSO is much less affected. 




    \item \underline{\textsf{epinions}}. For this benchmark, the conclusion 
    was more fine-grained --- both \confSU and \confSO were determined to perform
    better than \confST for `heavy' queries (i.e., those with latencies in the 99th \%-ile or more),
    but were determined to perform poorer than \confST for `lighter' queries (latencies less than 90\%-ile).
    This happens because in this benchmark there is high contention on locks yet also high number of atomic stores with release memory order. The speedup gained from the former and the slowdown incurred from the latter are both observed in this benchmark.

    \item \underline{Remaining benchmarks}. No statistically significant difference in performance between \confST, \confSU and \confSO could be determined for the remaining $6$ benchmarks.
    Their workloads have relatively low lock contention and low number of atomic releases for the overhead in vector clock computations to affect their performance. There is very little scope for improvement in these benchmarks with respect to vector clock computations.

\end{enumerate}
% While our algorithms do not unanimously significantly
% improve the performance of \confST, we performed a deeper dive to understand the gaps,
% and two important observations emerged.
% First, many of our benchmarks are I/O heavy (since they are database benchmarks)
% and often vector clock operations are only a tiny fraction of the
% total running time, making improvements in timestamping
% less evident.
% For this reason we also compared the overhead of non-sampling
% \tsan, namely \confT over the uninstrumented baseline \confNT
% to gauge the scope of improvement in timestamping (see Columns 2 and 3 in \tabref{tsan-throughputs}).
% Second, MySQL often makes heavy use of non-mutex synchronizations,
% such as atomic stores with release memory order, optimizing
% timestamping for which is beyond the scope of
% our current work. Here again, improvement in timestamping for lock based operations
% do not immediately yield performance improvements over \confST.
% We discuss these and other relevant details about our results next.

% \ucomment{First point out the diversity of workloads, and also queries within the workloads. Then go to Table1 and then discuss results there. Then say the thing about two-sample t-test.}



% After collecting the benchmark results in \tabref{tab:tsan}, we employed a two-sample t-test to determine whether the results for two different builds are significantly different at 5\% significance level. We grouped the observations into four categories:
% \begin{enumerate}
%     \item In the \textsf{sibench} and \textsf{ycsb} benchmarks, \textsf{sampling-u} and \textsf{sampling-o} performed better than \textsf{sampling-tsan}.
%     \item In the \textsf{tatp} and \textsf{twitter} benchmarks, \textsf{sampling-u} performed worse than \textsf{sampling-tsan}.
%     \item In the \textsf{epinions} benchmark, \textsf{sampling-u} and \textsf{sampling-o} performed worse than \textsf{sampling-tsan} for faster queries, but better for slower queries.
%     \item In the remaining benchmarks, there was no difference in performance with statistical significance among the three builds.
% \end{enumerate}


% There are various observations because (1) only some schema-workload pairs are heavily impacted by the cost of vector clock operations, and (2) some schema-workload pairs heavily use synchronizations based on atomic stores with release memory order which are not the key focus of this work. We discuss the insights in more detail below.

% We also show in \autoref{tab:tsan-throughputs} that MySQL Server suffered a huge slowdown when running with TSan as compared to running without TSan, whereas \textsf{sampling-tsan} incurred less slowdown because it handles less memory access events.


% \myparagraph{Time for VC operations is compounded for locks under high contention}{
% In \autoref{tab:tsan}, we observe a speedup in \textsf{sampling-u} and \textsf{sampling-o} for the \textsf{sibench} and \textsf{ycsb} benchmarks. Their workloads have multiple threads accessing the same table records at a high rate, causing high contention on their corresponding locks. The overhead of vector clock computations is compounded in this scenario. In turn, the speedup from our vector clock optimizations is also compounded.
% }

% \myparagraph{UTrack is not catered to atomic releases}
% {
% In \autoref{tab:tsan}, we observe a slowdown in \textsf{sampling-u} for the \textsf{tatp} and \textsf{twitter} benchmarks. Unlike \textsf{sibench} and \textsf{ycsb}, these benchmarks do not have high contention on locks and thus do not gain the compounded speedup. We profiled these benchmark executions and observed that there is a very high number of atomic stores with release memory order which introduces a large number of non-monotonic vector clocks updates.
% In our adaptation of \textsf{sampling-u} for such synchronizations, time spent in meta timestamp computations is longer than time saved from skipping computations. Such a slowdown is reasonable because the meta timestamp is designed for monotonic updates only. \textsf{sampling-o} is affected to a lesser degree.
% }

% \myparagraph{A mixture of high lock contention and high atomic releases}
% {
% In \autoref{tab:tsan}, we observe that for the \textsf{epinions} benchmark, there is a slowdown in \textsf{sampling-u} when considering the latency at the 90th percentile or lower (fast queries). However, there is a speedup in both \textsf{sampling-u} and \textsf{sampling-o} when considering the 99th percentile latency (slow queries) and the throughput. This happens because in this benchmark there is high contention on locks yet also high number of atomic stores with release memory order. The speedup gained from the former and the slowdown incurred from the latter are both observed in this benchmark.
% }

% \myparagraph{Workloads not impacted by overhead in vector clock computations}
% {
% In \autoref{tab:tsan}, the benchmarks not mentioned above do not show a difference in performance with statistical significance among the three builds. Their workloads have relatively low lock contention and low number of atomic releases for the overhead in vector clock computations to affect their performance. There is no scope for improvement in these benchmarks with respect to vector clock computations.
% }

\myparagraph{\rm \underline{\it \confSU v/s \confSO}}
{
For \textsf{ycsb}, \confSU performed better than \confSO by up to $1.36\times$ in latency and $1.04\times$ in aggregated throughput,
likely because the classic vector clock in \confSU benefited from cache optimizations, while our linked-list implementation in \confSO could have been optimized better.
However for \textsf{sibench} and \textsf{tatp}, \confSO performed better than \confSU by up to $1.66\times$ in latency and $1.17\times$ in aggregated throughput. We will discuss the effectiveness of \algoref{algo4} in finer detail through a controlled study in \secref{eval-rapid}.


% \myparagraph{Summary}{
% The vector clock optimizations in this work provide significant 
% performance improvements when there is high contention on locks. Furthermore, there can be future research on optimizations for synchronizations that perform non-monotonic vector clock updates.
% }





==> exec_macros.tex <==
%!TEX root = main.tex

% Drawing executions. Arguments: # of threads, and execution.
\newcommand{\execution}[2]{
\scalebox{0.85}{
  \begin{tikzpicture}%
    \foreach \x in {1,...,#1}
    \node[right] at (1.5*\x+0.2,0.25) {$t_{\x}$};
    \draw (1.2,0) -- (#1*1.5+1.3,0);%
    \pgfmathsetmacro{\y}{1};%
    #2%
    \draw (1.2,0) -- (1.2,-0.45*\y);%
    \draw (#1*1.5+1.3,0) -- (#1*1.5+1.3,-0.45*\y);%
    \foreach \x in {2,...,#1}
    % \draw[dashed] (1.5*\x-0.3,0) -- (1.5*\x-0.3,-0.4*\y);%
    \draw (1.2,-0.45*\y) -- (#1*1.5+1.3,-0.45*\y);%
  \end{tikzpicture}
}
}

% \figev arguments: thread id, event, variable/lock
\newcommand{\figev}[2]{
\pgfmathsetmacro{\y}{\y+1};
\pgfmathsetmacro{\y}{\y-1};
\node [left] at (1.25,-0.45*\y)  {\pgfmathprintnumber{\y}};%
\node at (#1*1.5 + 0.45,-0.45*\y) {$ #2 $};%
\pgfmathsetmacro{\y}{\y+1};
}

\newcommand{\figmev}[2]{
\pgfmathsetmacro{\y}{\y+1};
\pgfmathsetmacro{\y}{\y-1};
\node [left] at (1.25,-0.45*\y)  {\pgfmathprintnumber{\y}};%
\node[fill=blue!15!white] at (#1*1.5 + 0.45,-0.45*\y) {$ #2 $};%
\pgfmathsetmacro{\y}{\y+1};
}


\newcommand{\executionlarge}[2]{
\scalebox{0.85}{
  \begin{tikzpicture}%
    \foreach \x in {1,...,#1}
    \node[right] at (1.9*\x+0.2,0.25) {$t_{\x}$};
    \draw (1.2,0) -- (#1*1.9+1.9,0);%
    \pgfmathsetmacro{\y}{1};%
    #2%
    \draw (1.2,0) -- (1.2,-0.4*\y);%
    \draw (#1*1.9+1.9,0) -- (#1*1.9+1.9,-0.4*\y);%
    \foreach \x in {2,...,#1}
    % \draw[dashed] (1.5*\x-0.3,0) -- (1.5*\x-0.3,-0.4*\y);%
    \draw (1.2,-0.4*\y) -- (#1*1.9+1.9,-0.4*\y);%
  \end{tikzpicture}
}
}

% \figev arguments: thread id, event, variable/lock
\newcommand{\figevlarge}[2]{
\pgfmathsetmacro{\y}{\y+1};
\pgfmathsetmacro{\y}{\y-1};
\node [left] at (1.25,-0.4*\y)  {\pgfmathprintnumber{\y}};%
\node at (#1*1.9 + 0.45,-0.4*\y) {$ #2 $};%
\pgfmathsetmacro{\y}{\y+1};
}


% \figev arguments: thread id, event, variable/lock, 3rd arg = event id offset

% \newcommand{\mathresult}[1]{\pgfmathparse{#1} \pgfmathresult}
% \newcommand{\addmathresult}[1]{\pgfmathparse{2 *\mathresult{#1}} \pgfmathresult}

\newcommand{\figevoffset}[3]{
\pgfmathparse{#1}
\pgfmathsetmacro{\offset}{\pgfmathresult};
\pgfmathparse{\y+\offset}
\pgfmathsetmacro{\newindex}{\pgfmathresult};
\node [left] at (1.25,-0.4*\y)  {\pgfmathprintnumber{\newindex}};%
\node at (#2*1.5 + 0.45,-0.4*\y) {$ #3 $};%
\pgfmathsetmacro{\y}{\y+1};
}


%\orderedeg{t1}{ind1}{off1}{t2}{ind2}{off2} denotes an edge from an event e1
% to an event e2 such that ei appears at indi in the trace and belongs to thread ti.
% off1 and off2 are offsets from the center.
\newcommand{\orderedge}[6]{
  \draw[thick] (#1*1.5 + 0.45 + #3, -0.45*#2) edge[-{Latex[length=2mm, width=2mm]},  ->,>=stealth] (#4*1.5 + 0.45 + #6, -0.45*#5);
}

% The 7th arg is the label and the 8th argument is the position
\newcommand{\orderedgewithlabel}[8]{
  \draw (#1*1.5 + 0.45 + #3, -0.4*#2) edge[-{Latex[length=2mm, width=2mm]},  ->,>=stealth] node[anchor=center, sloped, #8] { #7} (#4*1.5 + 0.45 + #6, -0.4*#5);
}

\newcommand{\executionnonumber}[2]{
    \scalebox{0.85}{
        \begin{tikzpicture}%
        \foreach \x in {1,...,#1}
        \node[right] at (2*\x+0.5,0.25) {$t_{\x}$};
        \draw (1.9,0) -- (#1*2+1.6,0);%
        \pgfmathsetmacro{\z}{1};%
        #2%
        \draw (1.9,0) -- (1.9,-0.5*\z);%
        \draw (#1*2+1.6,0) -- (#1*2+1.6,-0.5*\z);%
        \foreach \x in {2,...,#1}
        \draw (2*\x-0.3,0) -- (2*\x-0.3,-0.5*\z);%
        \draw (1.9,-0.5*\z) -- (#1*2+1.6,-0.5*\z);%
        \end{tikzpicture}
    }
}                    

\newcommand{\figevnonumber}[2]{\node [left] at (1.75,-0.4*\z) {};%
% \node at (#1*1.5 + 0.45,-0.45*\y) {$ #2 $};%
\node [right] at (#1*2 + 0.3,-0.5*\z) {$ #2 $};%
\pgfmathsetmacro{\z}{\z+1};}

% Drawing programs. Arguments: # of threads, and program
\newcommand{\figprogram}[2]{\begin{tikzpicture}%
                              \foreach \x in {1,...,#1}
                                \node at (2.3*\x-1.15,0.25) {$t_{\x}$};
                              \draw (0,0) -- (#1*2.3+0.6,0);% 
                              \pgfmathsetmacro{\y}{1};%
                              #2%
                              \draw (0,0) -- (0,-0.4*\y);% 
                              \draw (#1*2.3+0.6,0) -- (#1*2.3+0.6,-0.4*\y);% 
                              \draw (0,-0.4*\y) -- (#1*2.3+0.6,-0.4*\y);% 
                            \end{tikzpicture}}
% figstmt arguments: thread id, offset, statement
\newcommand{\figstmt}[3]{\node [left] at (-0.15,-0.4*\y) {\pgfmathprintnumber{\y}};%
                      \node[right] at (#1*2.3 + #2*0.3 - 2.15,-0.4*\y) {\texttt{#3}};
                      \pgfmathsetmacro{\y}{\y+1};}

\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}



\newcommand{\nil}{\texttt{nil}}

\newcommand{\drawarrow}{\raisebox{2pt}{\scalebox{0.7}{\tikz{ \draw[-{Latex[length=2mm, width=2mm]},  ->,>=stealth](0,0) -- (7mm,0);} }}}

==> macros.tex <==
%!TEX root = main.tex

\makeatletter
\newcommand{\pnrelbar}{%
\linethickness{\dimen2}%
\sbox\z@{$\m@th\prec$}%
\dimen@=1.1\ht\z@
\begin{picture}(\dimen@,.4ex)
\roundcap
\put(0,.2ex){\line(1,0){\dimen@}}
\put(\dimexpr 0.5\dimen@-.2ex\relax,0){\line(1,1){.4ex}}
\end{picture}%
}

\newcommand{\precneq}{\mathrel{\vcenter{\hbox{\text{\prec@neq}}}}}
\newcommand{\prec@neq}{%
\dimen2=\f@size\dimexpr.04pt\relax
\oalign{%
\noalign{\kern\dimexpr.2ex-.5\dimen2\relax}
$\m@th\prec$\cr
\noalign{\kern-.5\dimen2}
\hidewidth\pnrelbar\hidewidth\cr
}%
}
\makeatother

\newenvironment{myparagraph}[1]{\vspace{0.1in}\noindent{\bf #1.}}{}

% \SetInd{0.3em}{0.2em}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{conjecture}[theorem]{Conjecture}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{problem}{Problem}
% \newtheorem{observation}{Observation}
\theoremstyle{remark}
\newtheorem*{remark}{Remark}


% Labels and references
\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\exlabel}[1]{\label{ex:#1}}
\newcommand{\exref}[1]{Example~\ref{ex:#1}}
\newcommand{\deflabel}[1]{\label{def:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\problabel}[1]{\label{prob:#1}}
\newcommand{\probref}[1]{Problem~\ref{prob:#1}}
\newcommand{\thmlabel}[1]{\label{thm:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\proplabel}[1]{\label{prop:#1}}
\newcommand{\propref}[1]{Proposition~\ref{prop:#1}}
\newcommand{\lemlabel}[1]{\label{lem:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\corlabel}[1]{\label{cor:#1}}
\newcommand{\corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\itmlabel}[1]{\label{itm:#1}}
\newcommand{\itmref}[1]{\ref{itm:#1}}
\newcommand{\equlabel}[1]{\label{eq:#1}}
\newcommand{\equref}[1]{Equation~(\ref{eq:#1})}
\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\applabel}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
% \newcommand{\appref}[1]{ the Appendix}
\newcommand{\algolabel}[1]{\label{app:#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{app:#1}}
\newcommand{\linelabel}[1]{\label{line:#1}}
\newcommand{\lineref}[1]{Line~\ref{line:#1}}
\newcommand{\linerangeref}[2]{Lines~\ref{line:#1}-\ref{line:#2}}
\newcommand{\secrangeref}[2]{Sections~\ref{sec:#1}-\ref{sec:#2}}

\newcommand{\rmv}[1] {}

\newcommand{\s}[1] {\mathsf{#1}}

\newcommand{\threads}[1]{\mathsf{Threads}_{#1}}
\newcommand{\locks}[1]{\mathsf{Locks}_{#1}}
\newcommand{\vars}[1]{\mathsf{Mem}_{#1}}
\newcommand{\events}[1]{\mathsf{Events}_{#1}}
\newcommand{\reads}[1]{\mathsf{Reads}_{#1}}
\newcommand{\writes}[1]{\mathsf{Writes}_{#1}}
\newcommand{\accesses}[1]{\mathsf{Accesses}_{#1}}
\newcommand{\acquires}[1]{\mathsf{Acquires}_{#1}}
\newcommand{\releases}[1]{\mathsf{Releases}_{#1}}
\newcommand{\forks}[1]{\mathsf{Forks}_{#1}}
\newcommand{\joins}[1]{\mathsf{Joins}_{#1}}
\newcommand{\match}[1]{\mathsf{match}_{#1}}
\newcommand{\lheld}[1]{\mathsf{locksHeld}_{#1}}

\newcommand{\eventset}{\mathfrak{E}}
\newcommand{\meventset}{\overline{\mathfrak{E}}}
\newcommand{\mevents}[1]{\mathsf{MkEvents}_{#1}}

\newcommand{\samprb}{Sampling Problem}
\newcommand{\analprb}{Analysis Problem}

\newcommand{\acq}{\mathtt{acq}}
\newcommand{\rel}{\mathtt{rel}}
\newcommand{\rd}{\mathtt{r}}
\newcommand{\wt}{\mathtt{w}}
\newcommand{\fork}{\mathtt{fork}}
\newcommand{\join}{\mathtt{join}}

\newcommand{\sync}{\mathtt{sync}}
\newcommand{\lk}{\ell}
% \newcommand{\ev}[1]{\langle #1\rangle}
\newcommand{\ev}[2]{{#2}^{#1}}
\newcommand{\tr}{\sigma}
\newcommand{\po}{\mathcal{P}}
\newcommand{\conf}{\asymp}
\newcommand{\comp}{\circ}
\newcommand{\EPO}{execution partial order }
\newcommand{\ThreadOf}[1]{\mathsf{thr}(#1)}
\newcommand{\ind}{\mathsf{index}}

%%%%%% trace parameters %%%%%%%
\newcommand{\trsz} {\s{N}}
\newcommand{\numthr} {\s{T}}
\newcommand{\numlk}{\s{L}}

\newcommand{\OpOf}[1]{\mathsf{op}(#1)}
\newcommand{\crit}[1]{\mathsf{CS}_{#1}}

%%%%%% substring etc. %%%%%%%%%

\newcommand{\ith}[2] {#1[#2]}
\newcommand{\substr}[3] {#1[#2,#3]}
\newcommand{\prefix}[2] {\substr{#1}{0}{#2}}
\newcommand{\suffix}[2] {\substr{#1}{#2}{\infty}}
\newcommand{\concat}{\circ}

\newcommand{\delequal}{\triangleq}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\setpred}[2]{\{#1 \,|\, #2\}}
\newcommand{\tuple}[1]{\langle #1 \rangle}

\DeclareFontFamily{U}{mathb}{\hyphenchar\font45}
\DeclareFontShape{U}{mathb}{m}{n}{
<5> <6> <7> <8> <9> <10> gen * mathb
<10.95> mathb10 <12> <14.4> <17.28> <20.74> <24.88> mathb12
}{}
\DeclareSymbolFont{mathb}{U}{mathb}{m}{n}
% \DeclareMathSymbol{\sqsubsetneq}    {3}{mathb}{"88}
% \DeclareMathSymbol{\varsqsubsetneq} {3}{mathb}{"8A}
% \DeclareMathSymbol{\varsqsubsetneqq}{3}{mathb}{"92}
\DeclareMathSymbol{\sqsubsetneq}    {3}{mathb}{"8A}

%% Acronyms
\newcommand{\acrtr}{\textsf{tr}\xspace}
\newcommand{\acrto}{\textsf{TO}\xspace}
\newcommand{\acrlk}{\textsf{LO}\xspace}
\newcommand{\acrconf}{\textsf{Conf}\xspace}
\newcommand{\acrhb}{\textsf{HB}\xspace}
\newcommand{\acrshb}{\textsf{SHB}\xspace}
\newcommand{\acrfhb}{\textsf{FHB}\xspace}
\newcommand{\acrchb}{\textsf{CHB}\xspace}
\newcommand{\acrcp}{\textsf{CP}\xspace}
\newcommand{\acrwcp}{\textsf{WCP}\xspace}
\newcommand{\acrsdp}{\textsf{SDP}\xspace}
\newcommand{\acrdc}{\textsf{DC}\xspace}
\newcommand{\ord}[2]{\leq^{#1}_{\mathsf{#2}}}
\newcommand{\notord}[2]{\not\leq^{#1}_{\mathsf{#2}}}
\newcommand{\strictord}[2]{<^{#1}_{\mathsf{#2}}}

\newcommand{\trord}[1]{\ord{#1}{\acrtr}}
\newcommand{\stricttrord}[1]{\strictord{#1}{\acrtr}}
\newcommand{\tho}[1]{\ord{#1}{\acrto}}
\newcommand{\stricttho}[1]{<^{#1}_{\acrto}}
\newcommand{\nottho}[1]{\not\leq^{#1}_{\acrto}}
\newcommand{\lko}[1]{\ord{#1}{\acrlk}}
\newcommand{\strictlko}[1]{<^{#1}_{\acrlk}}
\newcommand{\confo}[1]{\ord{#1}{\acrconf}}
\newcommand{\strictconfo}[1]{<^{#1}_{\acrconf}}
\newcommand{\hb}[1]{\ord{#1}{\acrhb}}
\newcommand{\stricthb}[1]{\strictord{#1}{\acrhb}}
\newcommand{\notstricthb}[1]{\not<^{#1}_{\acrhb}}


\newcommand{\lw}[1]{\mathsf{lw}_{#1}}
\newcommand{\proj}[2]{#1|_{#2}}

\newcommand{\ucomment}[1]{\textcolor{red}{#1}}
\newcommand{\mzcomment}[1]{\textcolor{blue}{MJ: #1}}
\newcommand{\mvcomment}[1]{\textcolor{green!70!black}{MV: #1}}
\newcommand{\dlcomment}[1]{\textcolor{orange}{DL: #1}}
% \newcommand{\ucomment}[1]{}
% \newcommand{\mzcomment}[1]{}
% \newcommand{\mvcomment}[1]{}
% \newcommand{\dlcomment}[1]{}

\newcommand\mycommfont[1]{\ttfamily{#1}}
% \newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}

\newcommand{\cre}{\mathsf{CR}}

\input{exec_macros}
\input{pseudocode_macros}

\renewcommand{\emptyset}{\varnothing}

\newcommand{\nats}{\mathbb{N}}
\newcommand{\rapid}{\textsf{RAPID}\xspace}
\newcommand{\pacer}{\textsc{Pacer}\xspace}
\newcommand{\RPT}{{\textsf{RPT}}\xspace}
\newcommand{\ProRace}{{\textsf{ProRace}}\xspace}
\newcommand{\TSVD}{{\textsf{TSVD}}\xspace}

\newcommand{\syncRPT}{{\bf\textsf{syncRPT}}\xspace}
\newcommand{\literace}{\textsc{LiteRace}\xspace}
\newcommand{\racemob}{\textsc{RaceMob}\xspace}

\newcommand{\pe}{\textsc{processed event}\xspace}
\newcommand{\raciness}{\text{raciness}\xspace}
\newcommand{\samplecost}{\textsc{sample cost}\xspace}
\newcommand{\distRPT}{{\bf\textsf{distRPT}}\xspace}

\newcommand{\djit}{\textsc{Djit}\xspace}
\newcommand{\djitp}{\textsc{Djit}+\xspace}
\newcommand{\fasttrack}{\textsc{FastTrack}\xspace}
\newcommand{\eraser}{\textsc{Eraser}\xspace}
\newcommand{\tsan}{\textsc{ThreadSanitizer}\xspace}

\newcommand{\mysql}{\textsc{MySQL Server}\xspace}

\newcommand{\vc}[1]{$\langle${\texttt{#1}}$\rangle$}

%% Table

\newcommand\VRule[1][\arrayrulewidth]{\vrule width #1}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

%%%

%%%%%%%%%% Macros for property tester %%%%%%%%

\newcommand{\hamd} {d_{\s{h}}}
\newcommand{\numsam} {r}
\newcommand{\samlen} {k}
\newcommand{\lh} {h}
\newcommand{\rcf} {\s{RF}}
\newcommand{\localindex}{\mathsf{threadIndex}}

%%% Macros for timestamps
\newcommand{\ft}{\mathsf{FT}}	% FastTrack
\newcommand{\smp}{\mathsf{sam}}	% Sample
\newcommand{\upd}{\mathsf{U}}	% Update
%% Local time
\newcommand{\ltime}{\mathsf{L}}
%% Causal time (should we call this global time? or epistemic time?)
\newcommand{\ctime}{\mathsf{C}}
\newcommand{\ltimeft}{{\ltime}_{\ft}}
\newcommand{\ctimeft}{{\ctime}_{\ft}}
\newcommand{\ltimesampling}{{\ltime}_{\smp}}
\newcommand{\ctimesampling}{{\ctime}_{\smp}}
\newcommand{\ltimefresh}{{\ltime}_{\upd}}
\newcommand{\ctimefresh}{{\ctime}_{\upd}}

% \newcommand{\algoname}{\textsc{FastTrack++}\xspace}
\newcommand{\algoname}{\textsc{UTrack}\xspace}

% Experiments
\newcommand{\confNT}{\textsf{NT}\xspace}
\newcommand{\confT}{\textsf{T}\xspace}
\newcommand{\confST}{\textsf{ST}\xspace}
\newcommand{\confSU}{\textsf{SU}\xspace}
\newcommand{\confSO}{\textsf{SO}\xspace}
\newcommand{\confET}{\textsf{ET}\xspace}
\newcommand{\confFT}{\textsf{FT}\xspace}

\newcommand{\confSTsr}[1]{\textsf{ST}\textsubscript{#1}}
\newcommand{\confSUsr}[1]{\textsf{SU}\textsubscript{#1}}
\newcommand{\confSOsr}[1]{\textsf{SO}\textsubscript{#1}}
\newcommand{\smpeng}[2]{{#1}-{(#2\%)}}
\newcommand{\SUThree}{\smpeng{\confSU}{3}\xspace}
\newcommand{\SOThree}{\smpeng{\confSO}{3}\xspace}
\newcommand{\SUFull}{\smpeng{\confSU}{100}\xspace}
\newcommand{\SOFull}{\smpeng{\confSO}{100}\xspace}


==> old-problem.tex <==
%TEX root=./main.tex

\ucomment{Maybe in the prelim we should define formally define the problem that \fasttrack solves. This way we will be able to contrast that one with this one.}

\ucomment{In the following, you are merely discussing existing sampling algorithms and their pros and cons. This is NOT what I was assuming you were doing. I had thought we were trying to show why existing sampling algorithms are just `instantiations' of the problem you just defined above. Doing this will illustrate that the problem you just defined is not out of the blue but actually captures all these existing works. I would suggest you rewrite the following part and go with the following structure:
\begin{enumerate}
	\item `Let us illustrate how the above problem captures the underlying problem being solved by existing sampling based approaches for race detection. As a consequence, an efficient and principled solution for \probref{race-detection-set} will likely yield more efficient solutions for each of these.'
	\item LiteRace. The LiteRace algorithm proposed by blah-blah-et-al [...] proposed an algorithm for race detection with the  guarantee that .... At a high level, it identifies these events by sampling x-many events randomly. Observe that by choosing $S$ to be a set constructed by randomly sampling each access event with ..., LiteRace precisely solves problem 1 above.
	\item PACER. Bond et al [...] ....
	\item RaceMob. ...
\end{enumerate}
}

Existing sampling approaches like \cite{bond2010pacer,popl2023,marino2009literace} usually firstly \ucomment{use `first' instead of `firstly'} decide $S$ using some sampling strategies and then analyze the sampled events in a way that is specific to strategies.
For example, \pacer split executions into alternative sampling and non-sampling phases. It samples all events in the sampling phase and in the non-sampling phase it only checks if the guesses it made in the sampling phases were correct.
In this way, the \pacer algorithm managed to reduce the majority of the cost on not only the read/write events but also the acquire/release events in the non-sampling phases. However, the \pacer algorithm's effectiveness relies heavily on its sampling strategy which requires that events are sampled in a "continuous" way. Achieving such a strategy it self can be expensive and outweighs the benefits.
\ucomment{This discussion about `continuous' can be postponed to next section or maybe a later part in this section. At this point, focus on demonstrating how well your problem statement can capture other algorithms.}
\ucomment{Start a new paragraph when starting new algorithm.} A similar example is the \RPT algorithm. \ucomment{What is the point of this empty sentence?}
\RPT is a property tester that make constant samples. It samples constantly many sub-traces of constant length. For each sampled trace, it runs \fasttrack.
For events(both read/write or acquires/release) not in the sampled sub-traces, it does nothing. While \RPT is extremely effective as it only analyzes constantly many events, it has the same restriction on $S$ as \pacer and its sampling strategy is expensive to implement online too.  
A different example would be literace. 
Effectively literace samples read/write events with some heuristics independently and analyzes all release/acquires as \fasttrack. Unlike \pacer or \RPT, the literace algorithm does not force $S$ to be unions of continuous events but at the same time it pays the same cost as a deterministic algorithm to all the release/acquires.


Sampling approaches generally get savings from two aspects: \ucomment{inline lists can be made using the latex command `\texttt{begin\{enumerate*\}}}' (a)analyzing less read/write events. (b)analyzing less acq/rel events. While the first part is relatively easy to achieve, the second part is more challenging as missing acquire/release events can result in computing a imcomplete HB \ucomment{Use the macro `\texttt{acrhb}' for good formatting} paritial order and thus lead to unsoundness. \pacer and \RPT manage to analyze less acq/req events at the cost of having an expensive sampling strategy. Literace on the hand fail to get any savings on these events as it made no assumptions on how $S$ was decided. 
Therefore, a natural question to ask is that can $S$ be an arbitrary small set of events and yet we can still soundly report all races of $S$ by without paying as much as a deterministic algorithm on all the acq/rel events? 





==> old-timestamp.tex <==
%!TEX root=./main.tex

\ucomment{old draft}\;
recall that the \fasttrack algorithm essentially computes timestamps that reflect the HB partial order of $\events{\tr}$. Now given that we only want to detect races over a restricted set $S\subset \events{\tr}$, we may not need to require the local time to reflect the full HB order. 
Before we present our technical details, let's understand how the \fasttrack timestamps computes the HB paritial order.  
At high level, the \fasttrack algorithm computes a local time $\ltimeft^\tr(e)$ and a vector timestamp $\ctimeft^\tr(e)$ for every event $e$ in a streaming manner.
As defined in \secref{prelim}, the local time $\ltimeft^\tr(e)$ of an event $e$ is the number of releases that have been performed in $\tr$ before $e$ by the same thread as $e$.  
The vector timestamp
$\ctimeft^\tr(e)$ captures $e$'s knowledge about the local time of other threads learned via HB edges. 

Note that two events from the same thread that are not separated by any release event will be assigned the same local time. The reason is that the two events are equivalent regarding the HB order. Similarly, events that are separated by any release event will be assigned different local time values as they are nonidentical in HB assuming that every release has a corresponding acquire. 

\fasttrack stores the local time of the last read and write accesses from each thread to each memory location. When a thread access a memory location, the algorithm checks for races by comparing the local time stored in the memory location against the thread's vector time stamp. 

Therefore, the local time of $e$ serves purely for purpose of for another thread to check if any event is not ordered with $e$ by HB.

In the case of sampling, the local time of event that is not sampled will not be stored into any memory location and therefore the local time of these event are non-relevant to the race detection procedure.

In another word, the local time only need to assign each sampled event a value and preserve the property of distinguishing two events from the same thread that are separated by any release of a lock. 
An easy way to achieve this is to ignore the "releases" that are non-relevant. 


Let's illustrate the idea with an simple example.
Consider the execution in \figref{motivating1}: $t_1$ in total has performed five events and only $e_1$, $e_4$ and $e_5$ are sampled. There are four releases of locks by $t_1$ and the \fasttrack timestamp will get incremented by four times(ends in $[5,0]$) after it processes events in stream. However, since $e_2$ and $e_3$ are not sampled, there is no benefit to distinguish them from other events, so the timestamp do not increase for release events $r_2$ and $r_3$. On the other hand, $e_1$ and $e_4$ must be assigned with different local time values (1 and 2) since events that are HB after $e_1$ may not be HB after $e_4$. 

The rough idea is that now only the first release after each sampled event "matters" and this defines a new time stamp. 
\input{algo2}
 \begin{align}
	\begin{array}{rcl}
    SR &=& \setpred{f}{\exists \lk,\OpOf{f} = \rel(\lk), \exists s (s\in S, f \text{ is the first release event such that } \ThreadOf{s}=\ThreadOf{f} }\\
    \ltimesampling^{(\tr,s)}(e) &=& |\setpred{f}{f\in SR, f \tho{\tr} e}|+1
	\end{array}
\end{align}

Similarly, we can define the corresponding vector time stamp
    \begin{align}
        \ctimesampling^{(\tr,s)}(e) = \lambda t \cdot \max \setpred{\ltimesampling{(\tr,s)}(f)}{\ThreadOf{f} = t, f \hb{\tr} e}
    \end{align}

As in the non-sampling case, the vector time stamp $ \ctimesampling^{(\tr,s)}(e)$ represents $e$'s knowledge about the events in other threads.

\algoref{algo2} presents a naive version of running \fasttrack on a sampled set $S$ that computes for each event $e$ the time stamp $\ctimesampling^{(\tr,s)}(e)$ . The algorithm is different from \algoref{djitp} in two places. In the release handler, now the local clock is incremented if the release is the first release after some sampled event. In the read/write handler, the algorithm only writes into the memory location if the event is sampled. 
Note that the algorithm nevertheless handles all acquire and release events with order $O(t)$ operations so it has the same running time complexity just as \fasttrack. 
However, if we consider the total time of changes on all the entries of any vector clock, it certainly have a smaller bound.
First observe that for every $e$. $\ltimesampling(e)$ is always bounded by the number of samples $\ThreadOf{e}$ made. Similarly $\sum \ctimesampling^{(\tr,s)}(e)$ is therefore bounded by $|S|$. 

Therefore, it's reasonable to assume that redundant operations(different releases of the same thread pass the same information) will occur. To further improve the algorithm, we introduce the second time stamp:


Let $\text{diff}(e_i,e_j)$ capture the number of different entries of the vector times of two events:
 \begin{align}
 \text{diff}(e_i,e_j)=|\{k|\ctimesampling^{(\tr,s)}(e_i)
 (k)\neq\ctimesampling^{(\tr,s)}(e_j)(k)\}|
 \end{align}
let $\text{next}(e)$ denote the succeeding event of $e$ in the same thread, if there is no such event, let $\text{next}(e)=e$.
now we can define $\text{VT}(e)$ as the following:
  \begin{align}
 \text{VT}(e)=\sum\text{diff}(e',\text{next}(e'))|e'\trord{\tr}e
 \end{align}

In essence, $\text{VT}(e)$ is a specific time stamp designed for the vector clock algorithms to reflect the number of times $C_{\ThreadOf{e}}$ change states before $e$ is processed. 

Similarly, we can define the vector time version of  $\text{VT}(e)$ as:    \begin{align}
        \text{U}(e) = \lambda t \cdot \max \setpred{\text{VT}(f)}{\ThreadOf{f} = t, f \hb{\tr} e}
    \end{align}



In the case of sampling, a thread $t$'s state may remain unchanged for multiple releases and other threads therefore may receive the same information from $t$ along different acquires of locks. In an algorithm which computes both time stamps, one may certainly use the $\text{U}$ clock to avoid vector clock operations after receiving the same information.


Let's illustrate how this time stamp can help us reduce redundant operations with an example. \ucomment{add example later}. 



\algoref{smp-upd} further optimizes \algoref{algo2} by computing the both time stamps for each event. Every thread and lock object now is assigned an additional U vector clock in addition to the S vector clock. The lock objects also record the thread ID of the threads that last release them.  
In the release handler, the lock $l$ checks if it already knows of the thread $t$ that is performing the release by comparing the U clocks. 
If it does not know of $t$, the lock copies both of the vector clocks and in both cases, the lock update $t$ as the thread that last releases it.  If the release happens to be the first release after a sampled event in $t$, it increments both of clocks. 
In the acquire handler, the thread checks if it knows of the thread that last releases the lock by comparing the U clocks. if it knows of it already, it simply skips the operation. Otherwise, the thread first performs a join of its U clock with the lock's U clock, and then it performs another join of its C clock with the lock's C clock. In the second join, the thread increments the local U clock by one for each entry changed. 
\ucomment{add lemmas and threoms for the correctness of the algorithm}


Unlike \algoref{algo2}, \algoref{smp-upd} results in a different running time complexity from \fasttrack. To see why this is the case we simply need to look into when the $O(|T|)$ operations are happening. 
In the acquire handler, the join operations happen when the guard $\CUpd_\lk(\lastrelthr_\lk) > \CUpd_t(\lastrelthr_\lk)$ fails. Recall that the local U clock $U_t[t]$ captures the number of times $C_t$ changes and is hence bounded by $|S|$. 
For a thread $t$, the the guard may fail for at most $|S|*|T|$ times(as the entries are monotonically growing). Since there are $|T|$ threads, we may therefore conclude that there are at most $|S|*|T|^2$ many $O(|T|)$ operations from the acquires. 
Similarly, in the release handler, the number of times a (monotone) copy will occur only when the guard $\CUpd_t(t) \neq \CUpd_\lk(t)$ fails. For each lock, the guard may fail $|S|*|T|$ times and therefore we may conclude that the total number of $O(|T|)$ operations from the releases is bounded by 
$O(|S||T||L|$.  Thus the total running time complexity of \algoref{smp-upd} is $O(n)+O(|S||T|^3)+O(|S||T|^2|L|)$.


There are two more observations worth discussing:(a) one may wonder if the causal time stamp $\ltimesampling$ itself can be used to reduce redundant operations. We note that this will result in unsoundness as the local time is not sufficient to reflect the "freshness" of the local clock. (b) we also note that the two local times can't not be merged into one. This is a crucial point for the algorithm to work. \ucomment{add examples}. 

Yet \algoref{smp-upd} still suffers from two problems. 
(a) The algorithm does not leverage all the advantages of the $VT$ time stamp. Notice that in an acquire, the $U$ clock informs the threads not only if they need to learn from other threads, but also how many entries they may need to update.

In \algoref{smp-upd}, the thread will perform a $O(t)$ join operations anyway even when $\CUpd_\lk(\lastrelthr_\lk)$ and $\CUpd_t(\lastrelthr_\lk)$ are off by one, which suggests that at most on entry needs to be updated. (b) The total $O(t)$ operations from the releases result in a sub term of $O(|S||T|^2|L|)$ in the running time complexity. In practices the number of locks can be much bigger than the number of threads. There are also synchronizations handled as lock-acquires/releases (accesses to volatile and atomic variables, barriers, wait and etc \cite{fasttrack}) which makes the term even more undesirable. In the next section, we will discuss how each of the issues can be conquered.

\input{algo-orderedlist.tex}

==> pseudocode_macros.tex <==
%!TEX root = ./main.tex

%%%%%% Macros for algo %%%%%%%%
\SetKwProg{myfun}{function}{}{}
\SetKwProg{myhandler}{handler}{}{}
\SetKwFunction{init}{initialize}
% \SetKwFunction{initClks}{InitClocks}
\SetKwFunction{preaccess}{preHandler}

% \SetKwFunction{reset}{resetData}
\SetKwFunction{resetClks}{resetClocksToNull}
\SetKwFunction{checkAndUpdate}{checkRaceAndUpdateMetadata}
\SetKwFunction{shouldSample}{shouldSample}
\SetKwFunction{newSample}{startNewSample}
\SetKwFunction{checkEndSample}{postHandler}

\SetKwFunction{endSample}{shouldEndSample}
\SetKwFunction{inSample}{inLocalSample}
\SetKwFunction{decidesampling}{decideSampling}
\SetKwFunction{skipevent}{returnWithoutInvokeEventHandler}

\SetKwFunction{merge}{mergeSubtraces}
% \SetKwFunction{fixpoint}{ComputeLCClosure}
\SetKwFunction{fixpoint}{ComputeSPIdeal}
\SetKwFunction{maxLB}{maxLowerBound}
\SetKwFunction{checkRace}{checkRace}
\SetKwFunction{rdhandler}{read}
\SetKwFunction{wthandler}{write}
\SetKwFunction{acqhandler}{acquire}
\SetKwFunction{relhandler}{release}
\SetKwInput{Params}{Parameters}
\SetKwInput{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKw{Let}{let}
\SetKw{Break}{break}
\SetKw{NOT}{not}
\SetKw{declare}{declare}
\SetKw{check}{check}
\SetKw{exit}{exit}
\SetKwFor{Foreach}{for each}{}{}%
\DontPrintSemicolon
% \newcommand{\ideal}{\mathsf{I}}
\renewcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}

\newcommand{\mx}{\sqcup}
\newcommand{\cle}{\sqsubseteq}

% \newcommand{\CFT}{\mathbb{C}^{\ft}}
% \newcommand{\RFT}{\mathbb{R}^{\ft}}
% \newcommand{\WFT}{\mathbb{W}^{\ft}}
\newcommand{\CFT}{\mathbb{C}}
\newcommand{\RFT}{\mathbb{C}^{\rd}}
\newcommand{\WFT}{\mathbb{C}^{\wt}}
% \newcommand{\CSmp}{\mathbb{C}^{\smp}}
% \newcommand{\RSmp}{\mathbb{R}^{\smp}}
% \newcommand{\WSmp}{\mathbb{W}^{\smp}}
\newcommand{\CSmp}{\mathbb{C}}
\newcommand{\COmp}{\mathbb{O}}
\newcommand{\epch}{\mathbbmss{e}}

\newcommand{\OL}{\mathbb{OL}}

\newcommand{\RSmp}{\mathbb{S}^{\rd}}
\newcommand{\WSmp}{\mathbb{S}^{\wt}}
\newcommand{\lastrelthr}{{\sf LR}}
% \newcommand{\CUpd}{\mathbb{C}^{\upd}}
\newcommand{\CUpd}{\mathbb{U}}
\newcommand{\lastrelu}{{\sf U}}



% \newcommand{\Ll}{\mathbb{L}}
% \newcommand{\LW}{\mathbb{LW}}



\newcommand{\On}{\mathbb{ON}}
\newcommand{\Off}{\mathbb{OFF}}
\newcommand{\phaseEnded}{\mathbb{EP}}
\newcommand{\nextEven}{\mathsf{nextEven}}
\newcommand{\update}{\mathsf{shouldUpdateEnd}}
\newcommand{\tid}{\mathsf{threadID}}
\newcommand{\clockVal}{\mathsf{clockValue}}
\newcommand{\shared}{\mathsf{shared}}

\newcommand{\sample}{\mathsf{isSampling}}
\newcommand{\globalsample}{\mathsf{globalSampleFlag}}
\newcommand{\localcounter}{\mathsf{localCounter}}
\newcommand{\globalphase}{\mathsf{globalSamplePhase}}
\newcommand{\localphase}{\mathsf{localSamplePhase}}


\newcommand{\checkR}{\mathsf{CheckedR}}
\newcommand{\checkW}{\mathsf{Checked}}

\renewcommand{\nil}{\mathtt{NIL}}
\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother
\newcommand{\apicall}[3]{{#1}\bigcdot{\textup{\texttt{#2(#3)}}}}
\newcommand{\first}[1]{\apicall{#1}{first}{}}
\newcommand{\removeFirst}[1]{\apicall{#1}{removeFirst}{}}
\newcommand{\isEmpty}[1]{\apicall{#1}{isEmpty}{}}
\newcommand{\lst}[1]{\apicall{#1}{last}{}}
\newcommand{\addLst}[2]{\apicall{#1}{addLast}{#2}}
\newcommand{\updateRel}[2]{\apicall{#1}{updateRelease}{#2}}

\newcommand{\true}{\top\!\!\!\!\top}
\newcommand{\false}{\bot\!\!\!\!\bot}


==> readwrite.tex <==
%!TEX root=./main.tex

\input{rwalgo}
\section{Read and Write events}
Algorithms~\ref{app:algo2}, \ref{app:smp-upd}, and~\ref{app:algo4} describe how the acquire and release handlers work to ensure that timestamps are maintained correctly to compute the sampling partial order $\hb{(\tr,S)}$. The last piece of the puzzle is to describe what the read and write handlers do and how race is detected. These are shown in \algoref{algo5}. The read and write handlers are almost the same as for {\fasttrack} with two important differences. First read and write clocks are updated only if the event belongs to $S$ (\lineref{read-sample} and \lineref{write-sample}). Second, suppose we observe an event $e \in S$ that accesses a variable $x$. To check if there is some later event $e'$ that is in race with $e$, we only need to check for race between $e$ and the first read/write events of each thread $t$. This is crucially exploited in \algoref{algo5}. Race is not checked at every data access event; only on the first in each thread after a new event is observed in $S$ (\lineref{rw-check}, \lineref{ww-check}, and \lineref{wr-check}). This ensures that the total number of race checks is bounded by $O(|S|\numthr)$ instead of $O(\trsz)$! Combining all these observations, we can observe that even after adding race checks, the total running time is still $O(\trsz) + O(|S|\numthr)O(\numthr)$.

\dlcomment{Formal statement about "algorithm detects a race in ... time and space"}

==> rwalgo.tex <==
%!TEX root = ./main.tex

{
\small
\begin{algorithm}[t]
% \BlankLine
\myfun{\init}{
	\ForEach{$t \in \threads{}$}{
		$\CUpd_t \gets \bot$ \;
		$\COmp_t \gets \bot$ \;
            $\shared_t\gets\false$\;
            $e_t\gets 1$

	}
	\ForEach{$x \in \vars{}$}{
		$\WFT_x \gets \bot$ \;
		$\RFT_x \gets \bot$
	}
 }
 \myhandler{\rdhandler{$t$, $x$}}{
        \If{$t$ hasn't checked race against latest $\wt(x)$-event in $S$ }{ \linelabel{rw-check}
        \lIf{$\WFT_x \not\cle \COmp_t$}{\declare race } 
        }
	
        \lIf{the event is sampled}{ \linelabel{read-sample}
           $\RFT_x\gets \RFT_x[t \mapsto e_t]$ 
        }

}


\myhandler{\wthandler{$t$, $x$}}{

     \If{$t$ hasn't checked race against latest $\wt(x)$-event in $S$ }{ \linelabel{ww-check}
        \lIf{$\WFT_x \not\cle \COmp_t$}{\declare race } 
        }
     \If{$t$ hasn't checked race against latest $\rd(x)$-event in $S$ }{ \linelabel{wr-check}
        \lIf{$\RFT_x \not\cle \COmp_t$}{\declare race } 
        }

    \If{the event is sampled}{ \linelabel{write-sample}
            \ForEach{$t' \in \threads{}$}{
            $\WFT_x\gets \WFT_x(t' \mapsto \COmp_t.\textbf{get}(t'))$
            }
        }
	
}



% \vspace*{0.25cm}
\caption{Read and Write handlers for Race detection}
\algolabel{algo5}
\end{algorithm}
}

==> sync-algo.tex <==
%!TEX root = ./main.tex

\small
\begin{algorithm}[t]
% \BlankLine
\myfun{\decidesampling}{
    $m \gets 4|T|+2h$ ;
    $\samlen \gets 4m/\epsilon$; 
    $\numsam \gets 15 \ln(1/\delta)/(2\epsilon)$ \;
    $\globalsample \gets \false$ \;
    $\globalphase \gets 0$ \;
    \For{$t \in \threads{\tr}$}{
        $I_t \gets$ Sample $\numsam$ indices in $[0,n_t-\samlen]$ \linelabel{rsample} \;
    }
}

\myfun{\preaccess{$t$, $o$}}{
    \If{$\Cc_t$ is $\bold{null}$}{
	    $\Cc_t \gets \bot[t \mapsto 1]$\;
        $\localphase_t \gets 0$ \;
        $\localcounter_t \gets 0$ \;
	}

    \If{$\localindex(t,o)\in I_t$}{
        $\globalsample \gets \true$ \;
        $\globalphase \gets \globalphase + 1$ \;
    }
    \If{$\localcounter_t>=\samlen$}{
        \If{$\globalphase=\localphase_t$}{
            $\globalsample \gets \false$ \;
        }
    }
    \If{$\localphase_t<\globalphase$}{
        $\localphase_t \gets \globalphase$ \;
        $\localcounter_t \gets 0$ \;
    }
    \If{$\globalsample$}{
        $\localcounter_t \gets \localcounter_t + 1$ \;
        \If{$o=\rd(x)\lor o=\wt(x)$}{
	    \lIf{$\Rr_x$ is $\bold{null}$}{
		    $\Rr_x \gets \bot$
	    }
	    \lIf{$\Ww_x$ is $\bold{null}$}{
		    $\Ww_x \gets \bot$
	    }
        }
        \If{$o=\acq(\lk)\lor o=\rel(\lk)$}{
	        \lIf{$\Ll_\lk$ is $\bold{null}$}{
		$\Ll_\lk \gets \bot$
	    }
         }
         \checkAndUpdate{$t,o,\localphase_t$} 
    
    }
    \Else{
        \skipevent \ucomment{\Return}
    }
}
\ucomment{Call the handler}
% \vspace*{0.25cm}
\caption{\textit{syncRPT}}
\algolabel{vc-updates}
\end{algorithm}

\normalsize

==> tables/latency_NT.tex <==
\begin{tabular}{lrrrrrrrrrr}
\toprule
           & auctionmark & epinions & hyadapt & seats & sibench & smallbank & tpcc & tpch & twitter & voter \\
\midrule
ST (0.3\%) & 1.02        & 2.32     & 1.62    & 1.84  & 0.16    & 1.08      & 0.69 & 4.15 & 2.18    & 0.39 \\
ST (3\%)   & 1.30        & 3.00     & 2.46    & 2.55  & 0.32    & 1.46      & 1.10 & 6.65 & 2.70    & 0.57 \\
ST (10\%)  & 1.57        & 2.81     & 4.13    & 3.32  & 0.54    & 1.72      & 1.67 & 7.92 & 3.99    & 0.82 \\
FT         & 1.92        & 6.19     & 26.30   & 4.38  & 1.01    & 1.96      & 2.44 & 10.04 & 6.88   & 1.28 \\
\bottomrule
\end{tabular}

==> tables/tsan-backup.tex <==
%!TEX root=../main.tex


\begin{table}
    \begin{tabular}{l|l|l|l|l|l|l|l|l}
        \hline
        & \textbf{BM} & \textbf{Min} & \textbf{25th} & \textbf{50th} & \textbf{75th} & \textbf{90th} & \textbf{99th} & \textbf{TP} \\
        \hline

        1 & \textsf{sibench} & & & & & & & \\
        & \textsf{ST} & $555\pm21$ & $23k\pm2k$ & $85k\pm4k$ & $140k\pm7k$ & $188k\pm13k$ & $539k\pm289k$ & $607\pm68$ \\
        & \textsf{SU} & $556\pm18$ & $22k\pm1k$ & $74k\pm3k$ & $123k\pm5k$ & $170k\pm13k$ & $560k\pm370k$ & $662\pm85$ \\
        & \textsf{SO} & $541\pm23$ & $22k\pm2k$ & $75k\pm4k$ & $124k\pm7k$ & $170k\pm16k$ & $506k\pm211k$ & $664\pm80$ \\
        \hline

        2 & \textsf{ycsb} & & & & & & & \\
        & \textsf{ST} & $412\pm5$ & $2.5k\pm434$ & $5.2k\pm524$ & $9.4k\pm706$ & $15k\pm1k$ & $57k\pm12k$ & $7.3k\pm542$ \\
        & \textsf{SU} & $414\pm3$ & $1.2k\pm75$ & $1.9k\pm137$ & $3.3k\pm249$ & $6.4k\pm384$ & $44k\pm5k$ & $14k\pm2k$ \\
        & \textsf{SO} & $408\pm4$ & $1.3k\pm114$ & $2.3k\pm200$ & $4.3k\pm333$ & $7.7k\pm438$ & $39k\pm6k$ & $13k\pm1k$ \\
        \hline

        
        3 & \textsf{tatp} & & & & & & & \\
        & \textsf{ST} & $496\pm8$ & $877\pm18$ & $1046\pm38$ & $1655\pm79$ & $14k\pm708 $& $58k\pm8k$ & $12k\pm1k$ \\
        & \textsf{SU} & $500\pm8$ & $890\pm20$ & $1063\pm36$ & $1689\pm69$ & $14k\pm708 $& $58k\pm8k$ & $12k\pm1k$ \\
        & \textsf{SO} & $494\pm10$ & $854\pm15$ & $1009\pm21$ & $1574\pm35$ & $14k\pm763$ & $55k\pm10k$ & $13k\pm1k$ \\
        \hline

        4 &\textsf{twitter} & & & & & & & \\
        & \textsf{ST} & $759\pm37$ & $363k\pm38k$ & $519k\pm65k$ & $737k\pm0.1M$ & $1M\pm0.2M$ & $1.6M\pm0.3M$ & $108\pm14$ \\
        & \textsf{SU} & $808\pm42$ & $437k\pm40k$ & $634k\pm68k$ & $891k\pm0.1M$ & $1.2M\pm0.2M$ & $1.9M\pm0.3M$ & $90\pm11$ \\
        & \textsf{SO} & $756\pm45$ & $360k\pm34k$ & $514k\pm57k$ & $712k\pm94k$ & $0.9M\pm0.1M$ & $1.5M\pm0.2M$ & $112\pm14$ \\
        \hline


        5 & \textsf{epinions} & & & & & & & \\
        & \textsf{ST} & $523\pm17$ & $1048\pm26$ & $1340\pm38$ & $3158\pm351$ & $1.7k\pm8k$ & $820k\pm75k$ & $1.8k\pm215$ \\
        & \textsf{SU} & $531\pm24$ & $1124\pm26$ & $1466\pm46$ & $3392\pm271$ & $20k\pm15k$ & $530k\pm28k$ & $2.4k\pm311$ \\
        & \textsf{SO} & $512\pm14$ & $1059\pm14$ & $1351\pm24$ & $3183\pm423$ & $15k\pm2.6k$ & $560k\pm70k$ & $2.4k\pm381$ \\
        \hline


        6 & \textsf{auctionmark} & & & & & & & \\
        & \textsf{ST} & $91\pm2$ & $1.9k\pm39$ & $5.1k\pm1k$ & $91k\pm18k$ & $316k\pm99k$ & $1.6M\pm0.7M$ & $543\pm168$ \\
        & \textsf{SU} & $91\pm3$ & $1.9k\pm31$ & $4.7k\pm1k$ & $90k\pm16k$ & $307k\pm76k$ & $1.6M\pm0.5M$ & $513\pm124$\\
        & \textsf{SO} & $92\pm2$ & $1.9k\pm23$ & $5.1k\pm1k$ & $90k\pm23k$ & $301k\pm0.1M$ & $1.4M\pm0.8M$ & $604\pm182$ \\
        \hline

        7 & \textsf{seats} & & & & & & & \\
        & \textsf{ST} & $115\pm5$ & $19k\pm4k$ & $94k\pm37k$ & $220k\pm89k$ & $413k\pm0.2M$ & $1.2M\pm0.3M$ & $385\pm113$ \\
        & \textsf{SU} & $117\pm4$ & $19k\pm4k$ & $85k\pm35k$ & $200k\pm84k$ & $392k\pm0.1M$ & $1.2M\pm0.4M$ & $389\pm124$ \\
        & \textsf{SO} & $113\pm5$ & $18k\pm4k$ & $94k\pm41k$ & $227k\pm102k$ & $434k\pm0.2M$ & $1.2M\pm0.4M$ & $385\pm126$ \\
        \hline

        8 & \textsf{smallbank} & & & & & & & \\
        & \textsf{ST} & $1363\pm60$ & $14k\pm1k$ & $24k\pm1k$ & $38k\pm3k$ & $70k\pm13k$ & $273k\pm0.1M$ & $1657\pm217$ \\
        & \textsf{SU} & $1366\pm65$ & $13k\pm1k$ & $23k\pm1k$ & $36k\pm2k$ & $63k\pm10k$ & $205k\pm0.1M$ & $1774\pm243$ \\
        & \textsf{SO} & $1322\pm65$ & $13k\pm1k$ & $23k\pm2k$ & $37k\pm4k$ & $64k\pm14k$ & $265k\pm80k$ & $1740\pm229$ \\
        \hline

        9 & \textsf{tpcc} & & & & & & & \\
        & \textsf{ST} & $100\pm5$ & $363k\pm16k$ & $687k\pm28k$ & $890k\pm60k$ & $1.1M\pm0.1M$ & $2.3M\pm1.1M$ & $89\pm8$ \\
        & \textsf{SU} & $103\pm5$ & $362k\pm18k$ & $685k\pm28k$ & $883k\pm63k$ & $1.1M\pm274k$ & $2.5M\pm2.3M$ & $89\pm12$ \\
        & \textsf{SO} & $101\pm5$ & $357k\pm13k$ & $677k\pm22k$ & $873k\pm49k$ & $1M\pm0.1M$ & $2M\pm0.6M$ & $92\pm6$ \\
        \hline

        10 & \textsf{voter} & & & & & & & \\
        & \textsf{ST} & $552\pm9$ & $16k\pm1k$ & $21k\pm974$ & $29k\pm2k$ & $57k\pm6k$ & $215k\pm65k$ & $1876\pm196$ \\
        & \textsf{SU} & $556\pm10$ & $16k\pm1k$ & $21k\pm860$ & $30k\pm2k$ & $57k\pm6k$ & $222k\pm107k$ & $1863\pm255$ \\
        & \textsf{SO} & $545\pm9$ & $16k\pm1k$ & $21k\pm994$ & $29k\pm1k$ & $54k\pm7k$ & $206k\pm55k$ & $1906\pm168$ \\
        \hline

        11 & \textsf{wikipedia} & & & & & & & \\
        & \textsf{T} & $672\pm31$ & $5k\pm215$ & $7499\pm1k$ & $40k\pm4k$ & $118k\pm23k$ & $722k\pm252k$ & $1208\pm276$ \\
        & \textsf{U} & $685\pm26$ & $5k\pm212$ & $7761\pm584$ & $4k\pm4k$ & $121k\pm25k$ & $710k\pm252k$ & $1167\pm267$ \\
        & \textsf{O} & $662\pm28$ & $5035\pm235$ & $7431\pm797$ & $39k\pm3k$ & $121k\pm22k$ & $742k\pm243k$ & $1190\pm242$ \\
    \end{tabular}
    \caption{Observation group 1 containing the sibench and ycsb benchmarks. Comparison of the throughput and latency of requests at various percentiles across configurations. Latency values are in microseconds. Throughput is the number of requests completed per second. All values are written in the form of mean $\pm$ standard deviation.}
    \label{tab:tsan}
\end{table}

==> tables/tsan-throughputs.tex <==
%!TEX root=../main.tex

\begin{table}
    \caption{Throughputs of no-tsan v/s tsan v/s sampling-t for all 11 benchmarks. Throughput is the number of requests completed per second, written in the form of mean $\pm$ standard deviation.}
    \scalebox{0.9}{
    \begin{tabular}{l l l l l l}
        1 & 2 & 3 & 4 & 5 & 6\\
        \hline
        \multirow{2}{*}{{\textbf{Benchmark}}} & \multicolumn{5}{c}{\textbf{Throughput (req/s)}} \\
        & \confNT & \confT & \confST & \confSU & \confSO \\
        \hline
        \textsf{auctionmark} & $606\pm217$ & $488\pm84$ & $543\pm168$ & $513\pm124$ & $604\pm182$  \\
        \textsf{epinions} & $19343\pm3236$ & $1080\pm133$ & $1760\pm215$ & $2399\pm311$ & $2336\pm227$ \\
        \textsf{seats} & $518\pm181$ & $170\pm15$ & $385\pm113$ & $389\pm124$ & $385\pm126$ \\
        \textsf{sibench} & $1200\pm222$ & $481\pm54$ & $607\pm68$ & $685\pm47$ & $802\pm33$ \\
        \textsf{smallbank} & $2651\pm860$ & $998\pm91$ & $1657\pm217$ & $1774\pm243$ & $1740\pm229$ \\
        \textsf{tatp} & $20495\pm3023$ & $9896\pm1121$ & $12406\pm1131$ & $11764\pm1733$ & $13379\pm2844$ \\
        \textsf{tpcc} & $162\pm33$ & $71\pm6$ & $89\pm8$ & $89\pm12$ & $92\pm6$ \\
        \textsf{twitter} & $2382\pm75$ & $58\pm2$ & $108\pm14$ & $90\pm11$ & $96\pm13$ \\
        \textsf{voter} & $2304\pm328$ & $1725\pm193$ & $1876\pm196$ & $1863\pm255$ & $1906\pm168$\\
        \textsf{wikipedia} & $1384\pm330$ & $1156\pm183$ & $1208\pm276$ & $1167\pm267$ & $1190\pm242$\\
        \textsf{ycsb} & $36924\pm4409$ & $6072\pm534$ & $7288\pm542$ & $14285\pm1993$ & $13688\pm1013$\\
        \hline
    \end{tabular}
    }
    \tablabel{tsan-throughputs}
\end{table}

==> tables/tsan.tex <==
%!TEX root=../main.tex


\begin{table}
    \caption{Evaluation of UTrack on MySQL benchmarks. Column 1 denotes benchmark names. Column 2 denotes the TSan configurations for each benchmark. Columns 3-7 show the various percentiles of the latency (time taken) of requests in microseconds. All values are written in the form of mean ${\pm}$ standard deviation.}
    \scalebox{0.9}{
    \begin{tabular}{l l l l l l l}
        1 & 2 & 3 & 4 & 5 & 6 & 7\\
        \hline & \\[-2ex]
        \multirow{2}{*}{{\textbf{Benchmark}}} & \multirow{2}{*}{{\textbf{Config}}} & \multicolumn{5}{c}{\textbf{Latency ($\mu$s)}}  \\
        & & \textbf{25 \%-ile} & \textbf{50 \%-ile} & \textbf{75 \%-ile} & \textbf{90 \%-ile} & \textbf{99 \%-ile} \\
        \hline & \\[-2ex]

        \multirow{3}{*}{{\textsf{auctionmark}}}
        & \confST & $1.9k{\pm}39$ & $5.1k{\pm}1k$ & $91k{\pm}18k$ & $316k{\pm}99k$ & $1.6M{\pm}0.7M$ \\
        & \confSU & $1.9k{\pm}31$ & $4.7k{\pm}1k$ & $90k{\pm}16k$ & $307k{\pm}76k$ & $1.6M{\pm}0.5M$ \\
        & \confSO & $1.9k{\pm}23$ & $5.1k{\pm}1k$ & $90k{\pm}23k$ & $301k{\pm}0.1M$ & $1.4M{\pm}0.8M$ \\
        \hline & \\[-2ex]

        \multirow{3}{*}{{\textsf{epinions}}}
        & \confST & $1.0k{\pm}26$ & $1.3k{\pm}38$ & $3.2k{\pm}351$ & $17k{\pm}8k$ & $820k{\pm}75k$ \\
        & \confSU & $1.1k{\pm}26$ & $1.5k{\pm}46$ & $3.4k{\pm}271$ & $15k{\pm}3.7k$ & $530k{\pm}28k$ \\
        & \confSO & $1.1k{\pm}16$ & $1.4k{\pm}38$ & $3.6k{\pm}265$ & $14k{\pm}1.4k$ & $559k{\pm}39k$ \\
        \hline & \\[-2ex]

        \multirow{3}{*}{{\textsf{seats}}}
        & \confST & $19k{\pm}4k$ & $94k{\pm}37k$ & $220k{\pm}89k$ & $413k{\pm}0.2M$ & $1.2M{\pm}0.3M$ \\
        & \confSU & $19k{\pm}4k$ & $85k{\pm}35k$ & $200k{\pm}84k$ & $392k{\pm}0.1M$ & $1.2M{\pm}0.4M$ \\
        & \confSO & $18k{\pm}4k$ & $94k{\pm}41k$ & $227k{\pm}102k$ & $434k{\pm}0.2M$ & $1.2M{\pm}0.4M$ \\
        \hline & \\[-2ex]

        \multirow{3}{*}{{\textsf{sibench}}}
        & \confST & $23k{\pm}2k$ & $85k{\pm}4k$ & $140k{\pm}7k$ & $188k{\pm}13k$ & $539k{\pm}289k$ \\
        & \confSU & $22k{\pm}1k$ & $74k{\pm}3k$ & $123k{\pm}5k$ & $170k{\pm}13k$ & $454k{\pm}118k$ \\
        & \confSO & $20k{\pm}312$ & $68k{\pm}870$ & $112k{\pm}2k$ & $148k{\pm}3k$ & $273k{\pm}74k$ \\
        \hline & \\[-2ex]

        \multirow{3}{*}{{\textsf{smallbank}}}
        & \confST & $14k{\pm}1k$ & $24k{\pm}1k$ & $38k{\pm}3k$ & $70k{\pm}13k$ & $273k{\pm}103k$ \\
        & \confSU & $13k{\pm}1k$ & $23k{\pm}1k$ & $36k{\pm}2k$ & $63k{\pm}10k$ & $205k{\pm}101k$ \\
        & \confSO & $13k{\pm}1k$ & $23k{\pm}2k$ & $37k{\pm}4k$ & $64k{\pm}14k$ & $265k{\pm}80k$ \\
        \hline & \\[-2ex]
        
        \multirow{3}{*}{{\textsf{tatp}}}
        & \confST & $877{\pm}18$ & $1046{\pm}38$ & $1655{\pm}79$ & $14k{\pm}708 $& $58k{\pm}8k$ \\
        & \confSU & $890{\pm}20$ & $1063{\pm}36$ & $1689{\pm}69$ & $15k{\pm}699 $& $62k{\pm}12k$ \\
        & \confSO & $862{\pm}14$ & $1017{\pm}18$ & $1588{\pm}33$ & $13k{\pm}262$ & $41k{\pm}3k$ \\
        \hline & \\[-2ex]

        \multirow{3}{*}{{\textsf{tpcc}}}
        & \confST & $363k{\pm}16k$ & $687k{\pm}28k$ & $890k{\pm}60k$ & $1.1M{\pm}0.1M$ & $2.3M{\pm}1.1M$ \\
        & \confSU & $362k{\pm}18k$ & $685k{\pm}28k$ & $883k{\pm}63k$ & $1.1M{\pm}274k$ & $2.5M{\pm}2.3M$ \\
        & \confSO & $357k{\pm}13k$ & $677k{\pm}22k$ & $873k{\pm}49k$ & $1M{\pm}0.1M$ & $2M{\pm}0.6M$ \\
        \hline & \\[-2ex]

        \multirow{3}{*}{{\textsf{twitter}}}
        & \confST & $363k{\pm}38k$ & $519k{\pm}65k$ & $737k{\pm}0.1M$ & $1M{\pm}0.2M$ & $1.6M{\pm}0.3M$ \\
        & \confSU & $437k{\pm}40k$ & $634k{\pm}68k$ & $891k{\pm}0.1M$ & $1.2M{\pm}0.2M$ & $1.9M{\pm}0.3M$ \\
        & \confSO & $434k{\pm}49k$ & $614k{\pm}75k$ & $802k{\pm}0.1M$ & $1M{\pm}0.1M$ & $1.7M{\pm}0.2M$ \\
        \hline & \\[-2ex]

        \multirow{3}{*}{{\textsf{voter}}}
        & \confST & $16k{\pm}1k$ & $21k{\pm}974$ & $29k{\pm}2k$ & $57k{\pm}6k$ & $215k{\pm}65k$ \\
        & \confSU & $16k{\pm}1k$ & $21k{\pm}860$ & $30k{\pm}2k$ & $57k{\pm}6k$ & $222k{\pm}107k$ \\
        & \confSO & $16k{\pm}1k$ & $21k{\pm}994$ & $29k{\pm}1k$ & $54k{\pm}7k$ & $206k{\pm}55k$ \\
        \hline & \\[-2ex]

        \multirow{3}{*}{{\textsf{wikipedia}}}
        & \confST & $5.1k{\pm}215$ & $7499{\pm}1k$ & $40k{\pm}4k$ & $118k{\pm}23k$ & $722k{\pm}252k$ \\
        & \confSU & $5.2k{\pm}212$ & $7761{\pm}584$ & $40k{\pm}4k$ & $121k{\pm}25k$ & $710k{\pm}252k$ \\
        & \confSO & $5.0k{\pm}235$ & $7431{\pm}797$ & $39k{\pm}3k$ & $121k{\pm}22k$ & $742k{\pm}243k$ \\
        \hline & \\[-2ex]

        \multirow{3}{*}{{\textsf{ycsb}}}
        & \confST & $2.5k{\pm}434$ & $5.2k{\pm}524$ & $9.4k{\pm}706$ & $15k{\pm}1k$ & $57k{\pm}12k$ \\
        & \confSU & $1.2k{\pm}75$ & $1.9k{\pm}137$ & $3.3k{\pm}249$ & $6.4k{\pm}384$ & $44k{\pm}5k$ \\
        & \confSO & $1.3k{\pm}107$ & $2.4k{\pm}200$ & $4.5k{\pm}333$ & $7.8k{\pm}438$ & $37k{\pm}2k$ \\
        \hline & \\[-2ex]
    \end{tabular}
    }
    \label{tab:tsan}
\end{table}

==> tree-clock.tex <==
%!TEX root=./main.tex

\section{Tree Clocks for Optimizing Cost of Timestamping}



==> tsan-changes.tex <==
%!TEX root=./main.tex

% \subsubsection{Adaptations for other synchronizations}

\algoref{smp-upd} and \algoref{algo4} were discussed under the context where the only synchronization mechanism is locking, in which every release follows an acquire by the same thread. In TSan, the acquire and release handlers also need to work for other synchronization mechanisms which may have different semantics. Below, we give the vector clock operation that is performed in TSan's implementation, some example use cases, and how to adapt our algorithms for them.

\myparagraph{\texttt{ReleaseStore}}
Vector clock copy. This is applied for operations such as mutex unlocking, atomic release-store, or thread forking. Both algorithms can be used as is, but \algoref{smp-upd} has to perform the full copy if the last acquire is not by the same thread (for correctly handling atomic release-store).

\myparagraph{\texttt{Release}}
Vector clock join. This is applied for operations such as unlocking of shared locks, barrier entries, or atomic read-modify-write (RMW) and compare-and-swap (CAS) operations within a release sequence. Both algorithms should perform a full vector clock or ordered list join.

\myparagraph{\texttt{Acquire}}
Vector clock join. This is applied for every acquire operation such as locking, atomic acquire-load or thread join. Both algorithms must perform a full copy of the vector clock (or ordered list) if the last release on the synchronization object was done by \texttt{Release}.

\myparagraph{\texttt{ReleaseAcquire}}
Vector clock copy followed by join. This is applied for RMW and CAS operations with acquire-release or sequentially-consistent memory order. For both algorithms, calling \texttt{ReleaseStore} followed by \texttt{Acquire} suffices.


